HaPy-Bug -- Human Annotated Python Bug Resolution Dataset

We present HaPy-Bug, a curated dataset of 793 Python source code commits associated with bug fixes, with each line of code annotated by three domain experts. The annotations offer insights into the purpose of modified files, changes at the line level, and reviewers' confidence levels. We analyze HaPy-Bug to examine the distribution of file purposes, types of modifications, and tangled changes. Additionally, we explore its potential applications in bug tracking, the analysis of bug-fixing practices, and the development of repository analysis tools. HaPy-Bug serves as a valuable resource for advancing research in software maintenance and security.

==> inside.tex <==
\hypertarget{introduction}{%
\section{1. Introduction}\label{introduction}}

\hypertarget{related-work}{%
\section{2. Related Work}\label{related-work}}

There is a number of interesting datasets that contain Python code
annotated with bug information. SecurityEval dataset
\cite{siddiq2022securityeval} contains automatically generated code. The
purpose of this dataset is a research on the vulnerability of such a
code. However, our dataset is more general as it contains code that
originates both from humans and machines.

Two other interesting datasets PySStuBs
\cite{DBLP:conf/msr/KamienskiPBH21} and TSSB-3M
\cite{DBLP:conf/msr/RichterW22} are devoted to the scrutiny of single
line/statement bugs. Although valuable such information is only partial.
However, our dataset contains annotations on both file- and line-level
giving a better insight into the process of bug emergence and
eradication.

The dataset BugsInPy \cite{DBLP:conf/sigsoft/WidyasariSLQPTT20} contains
a database of hundreds of bugs in Python code. We reference and use this
data set in our research. However, our dataset contains annotation on
both buggy and clean files and lines that allows for making balanced bug
detection datasets. It is rather thoroughly annotated Python code that
just bugs.

To summarize, in our opinion our proposed dataset is most multifaceted
and meticulous among existing bug-related Python code datasets. It
contains annotation for lines as well as files, for buggy as well as
clean code, for machine-generated and human-written code. Moreover, our
dataset contains all expert annotations and their confidence level, thus
proving insights in the annotation process, annotating experts and their
impact on the quality of annotations.

\hypertarget{data-collection}{%
\section{3. Data Collection}\label{data-collection}}

\hypertarget{annotation-process}{%
\section{4. Annotation Process}\label{annotation-process}}

The annotation process for this research adhered to a systematic
protocol designed to comprehensively analyze Python source code commits
linked to bug fixes. This procedure encompassed file categorization,
line annotation, project type identification, and reviewer confidence
assessments.

Annotators initiated the process by categorizing each file within a
commit into specific categories.

These categories included: ``programming'' covered source code files,
``tests'' included files dedicated to testing purposes, and
``documentation'' encompassed any form of documentation within the
project, ``project,'' which encompassed project management files that
may also contain source code, ``markup'' indicated files like HTML or
XML used as part of the project, and ``other'' served as a catch-all
category for files that did not fit the primary categories.

The next stage involved annotating lines within the files with specific
types of annotations. These annotations included ``bug(fix)'' for lines
related to bug identification or resolution and ``bug(fix) +
refactoring'' for lines combining bug fixes with code refactoring.
``Documentation'' annotations were used for lines containing
documentation. Lines associated with testing were annotated as ``test,''
while ``test + refactoring'' indicated lines involving test creation,
repair, or removal alongside code refactoring. ``Refactoring'' was
employed for lines featuring code changes that improved code readability
or structure without affecting system operation. ``Other'' annotations
were assigned to lines representing new functionality, other bug
entries, or updates of library/application versions for future
inclusion.

In addition to categorizing files and annotating lines, annotators also
annotated the type of project in which the bug was found. This
categorization was divided into three primary types: ``Bug in core
Python'' for issues within the core Python implementation, such as the
standard library; ``Bug in this Python application/library'' for bugs
occurring in applications or libraries primarily written in Python or
designed for Python; and ``Other'' for projects falling outside these
categories, including Python projects fixing dependencies or those with
Python scripts embedded in other languages.

To assess the reliability of annotations, annotators indicated their
confidence levels during the process. ``Confident reviewer'' (YES/NO)
signified the degree of confidence in the provided annotations, while
``Problematic'' (YES/NO) indicated whether any issues or challenges were
encountered during the annotation process. This comprehensive annotation
process ensured that the resulting dataset's annotations were accurate,
detailed, and valuable for subsequent analysis.

Six annotators with experience in Python programming, three of whom
possessed senior expertise, were engaged in the annotation process. The
distribution of bug resolutions among these annotators ensured that each
case was evaluated by at least three annotators.

The comprehensive annotation process adhered to the guidelines outlined
in the annotation protocol. Based on this protocol, 11 model annotations
were created, serving as a reference point for subsequent annotations.

After this, all annotators independently assessed and annotated the
assigned bug resolutions. Three annotators were tasked with evaluating
600 errors each, while the three more experienced annotators
collaboratively assessed 600 errors together, with each responsible for
marking 200 errors. This approach aimed to optimize the exposure of
senior annotators to a larger number of bugs.

This annotation process spanned a duration of two months. Weekly
meetings were held during this period, providing a platform for the
presentation and discussion of problematic bug reports. These sessions
facilitated the resolution of ambiguities and the establishment of
consensus on how to proceed in specific situations.

\begin{figure*}[p]
  \centering
  \includegraphics[width=0.915\textwidth]{infographics.pdf}
  % \caption{CVE lifetime characteristic and survival analysis.}
  % \label{fig:results}
\end{figure*}

\hypertarget{dataset-overview}{%
\section{5. Dataset Overview}\label{dataset-overview}}

\hypertarget{data-analysis}{%
\section{6. Data Analysis}\label{data-analysis}}

\hypertarget{applications}{%
\section{7. Applications}\label{applications}}

\begin{itemize}
\tightlist
\item
  Bug localization at file and line level - it can be used both to
  create a system ort to evaluate an existing system
\item
  Code Review Automation
\item
  Security Analysis
\item
  Best Practices and Coding Standards
\item
  Development of LLM models - this can be used to both for retraining
  and for evaluation
\end{itemize}

\hypertarget{limitations}{%
\section{8. Limitations}\label{limitations}}

\hypertarget{conclusion}{%
\section{9. Conclusion}\label{conclusion}}

\hypertarget{acknowledgments}{%
\section{10. Acknowledgments}\label{acknowledgments}}

\hypertarget{references}{%
\section{11. References}\label{references}}


==> table.tex <==
\begin{tabular}{lrrraaaaaaall}
\toprule
         &  \multicolumn{3}{c} {\bfseries Statistics} & \multicolumn{7} {a} {\bfseries Line annotations} &  \multicolumn{2} {c} {\bfseries Consensus}  \\
 Dataset &  Bugs &  Files &  Lines &  B &  B+R &  D &  O &  R &  T &  T+R &$=3$ &   $\geq 2$ \\

\midrule
bugs-in-py &   496 &   1382 &  20221 &     24.7\% &                    2.6\% &          13.2\% &   0.5\% &         1.9\% & 55.2\% &                1.9\% & 84.2\% &  97.8\% \\
     crawl &   145 &    759 &  26102 &     26.1\% &                    2.1\% &          29.2\% &   1.2\% &         1.5\% & 38.8\% &                1.2\% & 84.2\% &  98.7\% \\
       cve &   152 &    601 &  21640 &     29.6\% &                    2.2\% &          14.2\% &   1.2\% &         9.5\% & 42.0\% &                1.3\% & 81.5\% &  98.5\% \\
\bottomrule
\end{tabular}



